Self-adjointness for the MIT bag model on an unbounded cone

We consider the massless Dirac operator with the MIT bag boundary conditions on an unbounded three-dimensional circular cone. For convex cones, we prove that this operator is self-adjoint defined on four-component $H^1$--functions satisfying the MIT bag boundary conditions. The proof of this result relies on separation of variables and spectral estimates for one-dimensional fiber Dirac-type operators. Furthermore, we provide a numerical evidence for the self-adjointness on the same domain also for non-convex cones. Moreover, we prove a Hardy-type inequality for such a Dirac operator on convex cones, which, in particular, yields stability of self-adjointness under perturbations by a class of unbounded potentials. Further extensions of our results to Dirac operators with quantum dot boundary conditions are also discussed.

==> commands.tex <==
\newcommand\V{\mathbb{V}}
\newcommand{\xx}{{\boldsymbol{\mathsf{x}}}}
\newcommand\nb{\nabla}
\newcommand{\beq}{\begin{equation} \begin{split}}
\newcommand{\eeq}{\end{split} \end{equation}}
\newcommand\Sg{\Sigma}
\newcommand\Omg{\Omega}
\newcommand\ext{{\rm e}}
\newcommand\fru{u_\Omg}
\newcommand\avg[1]{\langle #1\rangle}

\makeatletter
\def\section{\@startsection{section}{1}\z@{.9\linespacing\@plus\linespacing}%
	{.7\linespacing} {\fontsize{13}{14}\selectfont\bfseries\centering}}
\def\paragraph{\@startsection{paragraph}{4}%
	\z@{0.3em}{-.5em}%
	{$\bullet$ \ \normalfont\itshape}}
\renewcommand\theequation{\thesection.\arabic{equation}}
\@addtoreset{equation}{section}
\makeatother


\newcommand{\dint}[2][]{\displaystyle{\int_{#2}^{#1}}}
\renewcommand\and{\qquad\text{and}\qquad}
\newcommand\as{\qquad\text{as}~}
\newcommand\sm{\setminus}
\newcommand\Op{\sfH_\omg^\Lambda}
\newcommand\Opf{\sfH_{\rm free}}
\newcommand{\Lii}[1]{L^2(\dR^{#1};\dC^{#1})}
\newcommand{\lii}[1]{L^2(\dR^{#1})}
\newcommand\frm{\frh_\omg^\Lambda}
\newcommand\frmD{\frh_{\omg, {\rm D}}^\Lambda}
\newcommand\frmf{\frh_{{\rm free}}}
\newcommand\frakm{\mathfrak{m}}
\newcommand\DtN{\sfL_\omg^\Lambda}
\newcommand\sfm{\mathsf{m}}
\newcommand\dtn{\wt{\sfL}_\omg^\Lambda}
\newcommand\Sol{\sfS_\Sigma}
\newcommand\Ev{\mu_\omg^\Lambda}
\newcommand\sinc{{\rm sinc}\,}
\newcommand\dl{\delta}
\newcommand\one{\mathbbm{1}}

\newcommand\Lm{\Lambda}
%\renewcommand\S{\Sigma}
%\newcommand\nb{\nabla}


\newcommand\first{the first representation theorem~\cite[Thm. VI 2.1]{Kato} }
\newcommand\trace{the trace theorem~\cite[Thm. 3.38]{McL} } 


\newcommand{\eq}{\\ & =}

\newcommand{\comm}[1]{}
\newcommand\lbra{\left}
\newcommand\rbra{\right}

\def\pp{{\prime}}
\def\dpp{{\prime\prime}}

\def\ddt#1{{\buildrel {\hbox{\LARGE ..}} \over {#1}}}   
\def\sfG{\mathsf{G}}
\def\sfSigma{\mathsf{\Sigma}}
\def\sfH{\mathsf{H}}\def\sfS{\mathsf{S}}
\def\sfS{\mathsf{S}}
\def\sfC{\mathsf{C}}
\def\bm1{\mathbbm{1}}
\def\G{\Gamma}
\def\C{\cC}
\def\g{\gamma}
\def\s{\sigma}
\def\sfh{\mathsf{h}}
\def\sfk{\mathsf{k}}
\def\p{\partial}
\def\sfw{\mathsf{w}}
\def\sfW{\mathsf{W}}
\def\one{\mathbbm{1}}
\def\omg{\omega}


\renewcommand{\iff}{\textit{if, and only if,}\,}

\newcommand{\spn}{\mathrm{span}\,}

\newcommand\myemph[1]{\textbf{\emph{#1}}} 
\def\Re{{\rm Re}\,}
\def\Im{{\rm Im}\,}

\def\arr{\rightarrow}

\def\medsum{{\textstyle\sum}}
\def\U{{\Upsilon}}
\def\diag{{\rm diag}\,}

\newcommand{\ee}{\mathsf{e}}
\newcommand{\zz}{\mathsf{z}}
\newcommand{\Ext}{{\rm Ext}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\Tt}{{\Theta}}
\renewcommand{\gg}{{\gamma}}
\def\m{\mathfrak{m}}
\def\tt{\theta}
\def\aa{\alpha}
\def\lm{\lambda}
\newcommand\sap{\sigma_{\rm ap}}

%\def\S{\Sigma}

%spectrum
\def\s{\sigma}
\def\sd{\sigma_{\rm d}}
\def\sess{\sigma_{\rm ess}}

\def\ii{{\mathsf{i}}}
\def\p{\partial} 

\def\pp{\prime}
\def\dpp{{\prime\prime}}
\def\tpp{{\prime\prime\prime}}

\def\kp{\kappa}

\def\sfH{\mathsf{H}}
\def\sfh{\mathsf{h}}
\def\one{\mathbbm{1}}
\def\Z{\mathsf{z}}
\def\sfP{\mathsf{P}}
\def\dd{{\mathsf{d}}}
\def\uhr{\upharpoonright}

\def\frf{{\mathfrak f}}
\def\frj{{\mathfrak j}}
\def\omg{\omega}


\def\sfw{\mathsf{w}}
\def\sfz{\mathsf{z}}


\def\sfS{\mathsf{S}}
\def\sfC{\mathsf{C}}
\def\sfW{\mathsf{W}}
\def\sfZ{\mathsf{Z}}
\def\sfP{\mathsf{P}}
\def\sfU{\mathsf{U}}
\def\sfV{\mathsf{V}}


\newcommand*{\medcap}{\mathbin{\scalebox{1.5}{\ensuremath{\cap}}}}%
\newcommand*{\medcup}{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}}%
\newcommand*{\medoplus}{\mathbin{\scalebox{1.5}{\ensuremath{\oplus}}}}%

\def\radius{3cm}
\def\softness{0.4}


\newcounter{counter_a}
\newenvironment{myenum}{\begin{list}{{\rm(\roman{counter_a})}}%
{\usecounter{counter_a}
\setlength{\itemsep}{1.ex}\setlength{\topsep}{0.8ex}
\setlength{\leftmargin}{5ex}\setlength{\labelwidth}{5ex}}}{\end{list}}
\newcommand\ds{\displaystyle}
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}



\newcommand{\eg}{{\it e.g.}\,}
\newcommand{\ie}{{\it i.e.}\,}
\newcommand{\cf}{{\it cf.}\,}

%--------------------------------
\numberwithin{figure}{section}
\numberwithin{equation}{section}
\theoremstyle{plain}% default
\newtheorem*{thm*}{Theorem}
\newtheorem{thm}{Theorem}[section]
\newtheorem{hyp}[thm]{Hypothesis}
\newtheorem{tm}{Theorem}%[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{example}[thm]{Example}
\newtheorem*{problem}{Open problem}

\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{notn}[thm]{Notation}
\newtheorem{calc}[thm]{Calculation}
\newtheorem*{thmA}{Theorem A}
\newtheorem*{thmB}{Theorem B}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{dfn}[thm]{Definition}
\theoremstyle{remark}
\newtheorem{remark}[thm]{Remark}
\theoremstyle{plain}
\newtheorem{hypothesis}{Hypothesis}
%--------------------------------

%
\newcommand{\dsp}{\displaystyle}
\newcommand{\spec}{{\mathrm{spec}}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rmi}{\mathrm{i}}
%\newcommand{\span}{\mathrm{span}\,}
\newcommand{\supp}{\mathrm{supp}\,}
\newcommand{\beu}{\begin{equation*}}
\newcommand{\eeu}{\end{equation*}}
\newcommand{\besu}{\begin{equation*}
\begin{aligned}}
\newcommand{\eesu}{\end{aligned}
\end{equation*}}
\newcommand{\bes}{\begin{equation}
\begin{aligned}}
\newcommand{\ees}{\end{aligned}
\end{equation}}

\newcommand\cA{\mathcal A}
\newcommand\cB{\mathcal B}
\newcommand\cD{\mathcal D}
\newcommand\cF{\mathcal F}
\newcommand\cG{\mathcal G}
\newcommand\cH{\mathcal H}
\newcommand\cK{\mathcal K}
\newcommand\cJ{\mathcal J}
\newcommand\cL{\mathcal L}
\newcommand\cM{\mathcal M}
\newcommand\cN{\mathcal N}
\newcommand\cP{\mathcal P}
\newcommand\cR{\mathcal R}
\newcommand\cS{\mathcal S}
\newcommand\CC{\mathbb C}
\newcommand\NN{\mathbb N}
\newcommand\RR{\mathbb R}
\newcommand\ZZ{\mathbb Z}
\newcommand\frA{\mathfrak A}
\newcommand\frB{\mathfrak B}
\newcommand\frS{\mathfrak S}
\newcommand\fra{\mathfrak a}
\newcommand\frq{\mathfrak q}
\newcommand\frs{\mathfrak s}
\newcommand\frp{\mathfrak p}
\newcommand\frh{\mathfrak h}
\newcommand\fraD{\mathfrak{a}_{\rm D}}
\newcommand\fraN{\mathfrak{a}}
\newcommand\eps{\varepsilon}
\newcommand\dis{\displaystyle}
\newcommand\ov{\overline}
\newcommand\wt{\widetilde}
\newcommand\wh{\widehat}
\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\eqdef}{=\mathrel{\mathop:}}
\newcommand{\defequ}{\mathrel{\mathop:}\hspace*{-0.72ex}&=}
\newcommand\vectn[2]{\begin{pmatrix} #1 \\ #2 \end{pmatrix}}
\newcommand\vect[2]{\begin{pmatrix} #1 \\[1ex] #2 \end{pmatrix}}
\newcommand\restr[1]{\!\bigm|_{#1}}
\newcommand\RE{\text{\rm Re}}

\newcommand\sign{{\rm sign\,}}


%\DeclareMathOperator\dom{dom}
%\DeclareMathOperator\ran{ran}

\newcommand\void[1]{}

\def\ov{\overline}
\def\eps{\varepsilon}
\def\ran{{\rm ran\,}}
\def\sigp{\sigma_{\rm p}}
\DeclareMathOperator\tr{tr}



%%%%

\def\sA{{\mathfrak A}}   \def\sB{{\mathfrak B}}   \def\sC{{\mathfrak C}}
\def\sD{{\mathfrak D}}   \def\sE{{\mathfrak E}}   \def\sF{{\mathfrak F}}
\def\sG{{\mathfrak G}}   \def\sH{{\mathfrak H}}   \def\sI{{\mathfrak I}}
\def\sJ{{\mathfrak J}}   \def\sK{{\mathfrak K}}   \def\sL{{\mathfrak L}}
\def\sM{{\mathfrak M}}   \def\sN{{\mathfrak N}}   \def\sO{{\mathfrak O}}
\def\sP{{\mathfrak P}}   \def\sQ{{\mathfrak Q}}   \def\sR{{\mathfrak R}}
\def\sS{{\mathfrak S}}   \def\sT{{\mathfrak T}}   \def\sU{{\mathfrak U}}
\def\sV{{\mathfrak V}}   \def\sW{{\mathfrak W}}   \def\sX{{\mathfrak X}}
\def\sY{{\mathfrak Y}}   \def\sZ{{\mathfrak Z}}

\def\frb{{\mathfrak b}}
\def\frl{{\mathfrak l}}
\def\frs{{\mathfrak s}}
\def\frt{{\mathfrak t}}



\def\dA{{\mathbb A}}   \def\dB{{\mathbb B}}   \def\dC{{\mathbb C}}
\def\dD{{\mathbb D}}   \def\dE{{\mathbb E}}   \def\dF{{\mathbb F}}
\def\dG{{\mathbb G}}   \def\dH{{\mathbb H}}   \def\dI{{\mathbb I}}
\def\dJ{{\mathbb J}}   \def\dK{{\mathbb K}}   \def\dL{{\mathbb L}}
\def\dM{{\mathbb M}}   \def\dN{{\mathbb N}}   \def\dO{{\mathbb O}}
\def\dP{{\mathbb P}}   \def\dQ{{\mathbb Q}}   \def\dR{{\mathbb R}}
\def\dS{{\mathbb S}}   \def\dT{{\mathbb T}}   \def\dU{{\mathbb U}}
\def\dV{{\mathbb V}}   \def\dW{{\mathbb W}}   \def\dX{{\mathbb X}}
\def\dY{{\mathbb Y}}   \def\dZ{{\mathbb Z}}

\def\sfA{{\mathsf A}}   \def\sfB{{\mathsf B}}   \def\sfC{{\mathsf C}}
\def\sfD{{\mathsf D}}   \def\sfE{{\mathsf E}}   \def\sfF{{\mathsf F}}
\def\sfG{{\mathsf G}}   \def\sfH{{\mathsf H}}   \def\sfI{{\mathsf I}}
\def\sfJ{{\mathsf J}}   \def\sfK{{\mathsf K}}   \def\sfL{{\mathsf L}}
\def\sfM{{\mathsf M}}   \def\sfN{{\mathsf N}}   \def\sfO{{\mathsf O}}
\def\sfP{{\mathsf P}}   \def\sfQ{{\mathsf Q}}   \def\sfR{{\mathsf R}}
\def\sfS{{\mathsf S}}   \def\sfT{{\mathsf T}}   \def\sfU{{\mathsf U}}
\def\sfV{{\mathsf V}}   \def\sfW{{\mathsf W}}   \def\sfX{{\mathsf X}}
\def\sfY{{\mathsf Y}}   \def\sfZ{{\mathsf Z}}


\def\cA{{\mathcal A}}   \def\cB{{\mathcal B}}   \def\cC{{\mathcal C}}
\def\cD{{\mathcal D}}   \def\cE{{\mathcal E}}   \def\cF{{\mathcal F}}
\def\cG{{\mathcal G}}   \def\cH{{\mathcal H}}   \def\cI{{\mathcal I}}
\def\cJ{{\mathcal J}}   \def\cK{{\mathcal K}}   \def\cL{{\mathcal L}}
\def\cM{{\mathcal M}}   \def\cN{{\mathcal N}}   \def\cO{{\mathcal O}}
\def\cP{{\mathcal P}}   \def\cQ{{\mathcal Q}}   \def\cR{{\mathcal R}}
\def\cS{{\mathcal S}}   \def\cT{{\mathcal T}}   \def\cU{{\mathcal U}}
\def\cV{{\mathcal V}}   \def\cW{{\mathcal W}}   \def\cX{{\mathcal X}}
\def\cY{{\mathcal Y}}   \def\cZ{{\mathcal Z}}


\def\N{\mathbb{N}}

\renewcommand{\div}{\mathrm{div}\,}
\newcommand{\grad}{\mathrm{grad}\,}
\newcommand{\Tr}{\mathrm{Tr}\,}

\newcommand{\dom}{\mathrm{dom}\,}
\newcommand{\mes}{\mathrm{mes}\,}
